Prompting ELECTRA: Few-Shot Learning with Discriminative Pre-Trained Models

Pre-trained masked language models successfully perform few-shot learning by formulating downstream tasks as text infilling. However, as a strong alternative in full-shot settings, discriminative pre-trained models like ELECTRA do not fit into the paradigm. In this work, we adapt prompt-based few-shot learning to ELECTRA and show that it outperforms masked language models in a wide range of tasks. ELECTRA is pre-trained to distinguish if a token is generated or original. We naturally extend that to prompt-based few-shot learning by training to score the originality of the target options without introducing new parameters. Our method can be easily adapted to tasks involving multi-token predictions without extra computation overhead. Analysis shows that ELECTRA learns distributions that align better with downstream tasks.

==> sections/concurrent.tex <==
\section{Concurrent Works}
Two concurrent works explore similar ideas to prompt discriminative pre-training models \cite{yao-etal-2022-prompt, li2022pre}. \citet{yao-etal-2022-prompt} propose an approach to prompting ELECTRA by concatenating the context and all the target words with an emphasis to show that prompting based learning outperforms standard fine-tuning on ELECTRA. Similar to \citet{li2022pre}, our work further discovers the advantage of discriminative pretrained models over masked language models on the few-shot prompt-based setting.

==> sections/related.tex <==
%!TEX root = ../main.tex

\section{Related Work}
Previous works mostly use prompt-base finetuning on models in low-compute scenarios \cite{schick2021exploiting, gao2021making, schick2021true} and zero-shot or few-shot priming for gigantic language models \cite{brown2020language, artetxe2021efficient, rae2021scaling}.

Generative-style language models suffer from surface form competition where sequences of similar meaning compete for probability masses. \citet{holtzman2021surface} reweights options by  considering its priori likelihood to compensates for the issue. \citet{min2021noisy} proposes a noisy channel approach to instead compute the conditional probability of the input given the label for more accurate and stable predictions.

 Recently, concurrent works demonstrate that fine-tuning gigantic autoregressive language models with a large number of tasks enables zero-shot generalization to unseen tasks \cite{sanh2022multitask, wei2022finetuned} and effectively reduces the gap between large and small models as the number of tasks increases \cite{xu2022zeroprompt}. Scaling up tasks also enables in-context learning for unseen tasks through meta-learning \cite{min2021metaicl, zhong2021adapting}.

While almost all the previous works focus on prompt-based learning with generative language models, our work explores adapting discriminative models for prompt-based few-shot learning.


==> tables/large_v2.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccc} \toprule
 & K  & BERT                 & RoBERTa & ELECTRA              \\ \midrule
SST-2     & 0  & 61.2                 & 83.6    & 86.0                 \\
          & 16 & 87.9                 & 93.0    & 93.6                 \\ \midrule
SST-5     & 0  & 25.7                 & 34.7    & 32.1                 \\
          & 16 & 42.4                 & 47.1    & 50.3                 \\ \midrule
BoolQ     & 0  & 49.3                 & 53.4    & 71.1                 \\
          & 16 & 56.9                 & 70.3    & 75.2                 \\\midrule
SNLI      & 0  & 41.5                 & 49.8    & 59.4                 \\
          & 16 & 60.6                 & 79.4    & 79.1                 \\ \bottomrule
\end{tabular}}
\caption{Prompt-based zero-shot and few-shot performance on RoBERTa-large and ELECTRA-large models. }
\label{tab:large_v2}
\end{table}

\section{Template Sensitivity}

\paragraph{Template Sensitivity} We conduct prompt-based few-shot finetuning with different templates and show results in \autoref{tab:template_sensitivity}. More template details are in \autoref{app:template}. ELECTRA consistently outperforms RoBERTa with different templates. \danqi{I really think it is quite bad to use $T_1$, $T_2$ and $T_3$ and they refer to different things for different tasks I assume? Either you detail the templates in some way, or I think what you only need is to show the average and standard deviation. It seems that the standard deviations are both small for RoBERTa and ELECTRA though. I suggest you remove the table from the main paper especially if space is a concern. Consider adding a subsection in appendix about this point.} \mikel{I agree that we can move this to an appendix if short in space}
\input{tables/template}


